Exploring Gamma-Ray Bursts, Their Immediate Environment and Host Galaxies

Lasting anywhere from a few milliseconds to several minutes, GRBs shine hundreds of times brighter than a typical supernova, making them briefly the brightest source of cosmic gamma-ray photons in the observable Universe. This thesis focuses on 3 different aspects of GRBs: (1) The radiative mechanism of GRBs and their afterglows, i.e. the occurrence of thermal emission and the physical parameters we can determine through this emission. (2) Their host galaxies, using results from observations of GRB 121024A as a case study. (3) How they can be used to answer some of the larger astrophysical questions, more specifically in this case, to study interstellar dust and grey extinction.

==> quote.tex <==
\vspace*{0.7\textheight}
\begin{flushright}
\noindent Our whole universe was in a hot dense state,\\
Then nearly fourteen billion years ago expansion started. Wait\dots\\
The Earth began to cool,\\
The autotrophs began to drool,\\
Neanderthals developed tools,\\
We built a wall (we built the pyramids),\\
Math, science, history, unraveling the mysteries,\\
That all started with the big bang!\dots\\
from "\textit{The Big Bang Theory}" -- Barenaked Ladies
\end{flushright}

